Evaluating and Optimizing the Effectiveness of Neural Machine Translation in Supporting Code Retrieval Models: A Study on the CAT Benchmark

Neural Machine Translation (NMT) is widely applied in software engineering tasks. The effectiveness of NMT for code retrieval relies on the ability to learn from the sequence of tokens in the source language to the sequence of tokens in the target language. While NMT performs well in pseudocode-to-code translation, it might have challenges in learning to translate from natural language query to source code in newly curated real-world code documentation/ implementation datasets. In this work, we analyze the performance of NMT in natural language-to-code translation in the newly curated CAT benchmark that includes the optimized versions of three Java datasets TLCodeSum, CodeSearchNet, Funcom, and a Python dataset PCSD. Our evaluation shows that NMT has low accuracy, measured by CrystalBLEU and Meteor metrics in this task. To alleviate the duty of NMT in learning complex representation of source code, we propose ASTTrans Representation, a tailored representation of an Abstract Syntax Tree (AST) using a subset of non-terminal nodes. We show that the classical approach NMT performs significantly better in learning ASTTrans Representation over code tokens with up to 36% improvement on Meteor score. Moreover, we leverage ASTTrans Representation to conduct combined code search processes from the state-of-the-art code search processes using GraphCodeBERT and UniXcoder. Our NMT models of learning ASTTrans Representation can boost the Mean Reciprocal Rank of these state-of-the-art code search processes by up to 3.08% and improve 23.08% of queries' results over the CAT benchmark.

==> content/Abstract_arxiv.tex <==
% Solving every Software Engineering task can be formulated as designing/ applying models to infer the target objects from input objects. In the scope of this paper, we call models constructed earlier in the history of approaches for solving a Software Engineering task  classical models, while those that appeared recently as modernized models. Modernized models usually have higher accuracy than classical models thanks to their better designation to deal with the complexity of target objects. In this work, we want to test whether classical models can learn better with the simplified version of target objects. If yes, we can propose a combined model that integrates the ability to learn output by classical models. In other words, while a modernized model learns the original target objects, a classical model is constructed to learn a simplified version of the target object and will be augmented as an extra input of the modernized model to enhance the accuracy of the modernized model.

% In this work, we implement this idea for an important software engineering task: code search with the input object as natural language description and the output object as source code snippets. In this task, GraphCodeBERT and uniXcoder are two modernized models, and we choose the classical model as the Neural Machine Translation model. Next, we design ASTTrans, our designed representation of source code, to simplify the target object for the classical model. Finally, we integrated the output as translated ASTTrans representation by the Neural Machine Translation model to be an extra input for code search with modernized models. By evaluation, we show how helpful the classical model performs in this scenario by the improvement of up to 3\% of code search over datasets of the CAT benchmark.
Solving every Software Engineering task involves designing or applying models to infer the target object from the source object. In this paper, we differentiate between classical models, which were developed earlier in the history of Software Engineering approaches, and modernized models, which have emerged more recently. Modernized models generally exhibit higher accuracy due to their improved ability to handle complex target objects.

The aim of this work is to investigate whether classical models can benefit from learning a simplified version of the target objects. If this proves to be the case, we propose a combined model that integrates the learning capabilities of classical models. In other words, while modernized models learn the original target objects, classical models are trained on simplified versions of the target object and their outputs are used as additional inputs to enhance the accuracy of the modernized models.

We apply this concept to the task of code search in Software Engineering. The source objects are natural language descriptions, and the target objects are source code snippets. For code search, we employ GraphCodeBERT and uniXcoder as modernized models, and the classical model we choose is the Neural Machine Translation model. To simplify the target object for the classical model, we design ASTTrans, a representation of the source code. The output of the Neural Machine Translation model, which translates the ASTTrans representation, is then integrated as an extra input for code search using the modernized models. Through evaluation, we demonstrate the effectiveness of the classical model in this context, achieving an improvement of up to 3\% Mean Reciprocal Rank in code search performance across datasets from the CAT benchmark.


==> content/Equations.tex <==
% https://latexeditor.lagrida.com/

% Query \space A_{1}
% \\
% Candidate \space B_{1}
% \\
% Candidate \space B_{2}
% \\
% Candidate \space B_{3}

% Org. Emb. of A_{1}: \space \overrightarrow{n}
% \\
% Org. Emb. of B_{1}: \space \overrightarrow{c_{1}}
% \\
% Org. Emb. of B_{2}: \space \overrightarrow{c_{2}}
% \\
% Org. Emb. of B_{3}: \space \overrightarrow{c_{3}}

% Aug. Emb. of A_{1}: \space \overrightarrow{n^{'}}
% \\
% Aug. Emb. of B_{1}: \space \overrightarrow{c^{'}_{1}}
% \\
% Aug. Emb. of B_{2}: \space \overrightarrow{c^{'}_{2}}
% \\
% Aug. Emb. of B_{3}: \space \overrightarrow{c^{'}_{3}}


% \\
% matrix\_sim_{org}=[[s_{1},s_{2},s_{3}]] 
% \\
% s_{1}=cosine\_sim(\overrightarrow{n},\overrightarrow{c_{1}})
% \\
% s_{2}=cosine\_sim(\overrightarrow{n},\overrightarrow{c_{2}})
% \\
% s_{3}=cosine\_sim(\overrightarrow{n},\overrightarrow{c_{3}})

% \\
% matrix\_sim_{org}=[[s_{1},s_{2},s_{3}]] 
% \\
% s_{1}=cosine\_sim(\overrightarrow{n},\overrightarrow{c_{1}})=0.9
% \\
% s_{2}=cosine\_sim(\overrightarrow{n},\overrightarrow{c_{2}})=0.8
% \\
% s_{3}=cosine\_sim(\overrightarrow{n},\overrightarrow{c_{3}})=0.5


% \\
% matrix\_sim_{aug}=[[s^{'}_{1},s^{'}_{2},s^{'}_{3}]] 
% \\
% s^{'}_{1}=cosine\_sim(\overrightarrow{n^{'}},\overrightarrow{c^{'}_{1}})
% \\
% s^{'}_{2}=cosine\_sim(\overrightarrow{n^{'}},\overrightarrow{c^{'}_{2}})
% \\
% s^{'}_{3}=cosine\_sim(\overrightarrow{n^{'}},\overrightarrow{c^{'}_{3}})

% matrix\_sim_{com}
% \\
% =matrix\_sim_{org}*(1-w)+matrix\_sim_{aug}*w
% \\
% d_{1}=s_{1}*(1-w)+s^{'}_{1}*w
% \\
% d_{2}=s_{2}*(1-w)+s^{'}_{2}*w
% \\
% d_{3}=s_{3}*(1-w)+s^{'}_{3}*w
 
% Top \space Candidates \space for A_{1}
% \\
% Top \space 1 = B_{2}
% \\
% Top \space 2 = B_{1}
% \\
% Top \space 3 = B_{3} 

% Top \space Candidates \space for A_{1}
% \\
% Top \space 1 = B_{1}
% \\
% Top \space 2 = B_{2}
% \\
% Top \space 3 = B_{3} 

==> content/ExperimentResult.tex <==
\section{Results}
\subsection{RQ1. NMT's Performance Evaluation.}
\input{figTabAlgs/tbl_rq1}
The result for RQ1 is shown in Table \ref{asttrans:rq1}. From the translated result of the test sets in four datasets, we see that the inference from query to code tokens confronts challenges for Neural Machine Translation. Due to large side vocabularies in the training sets, NMT got low accuracy measured by both the Crystal-BLEU-4 and Meteor scores. The best dataset for Query-to-Code Tokens translation is TLC, with the scores with a Crystal-BLEU-4 score of 0.16. This dataset included over 400000 distinct tokens in their training set of 53592 candidates. Similarly, other datasets in the Java language as CSN and Funcom or the Python dataset PCSD, also achieved low scores both by Crystal-BLEU-4 and Meteor, which confirmed our hypothesis that source code candidates are too complicated for the NMT model to learn their information, unlike manually curated datasets for pseudocode-to-code translation such as SPOC \cite{025_SPoC}.

While Query-to-Code Tokens got low accuracy by NMT translation, Table \ref{asttrans:rq1} also shows that Query-to-ASTTrans Representation achieved much better accuracy. Consistent with learning the terminal nodes of AST, the NMT model to learn the sequence of non-terminal nodes achieved the highest accuracy in translation of the TLC dataset, while it got the lowest accuracy on the CSN dataset. Comparing by the ratio, the NMT can perform about three times better on learning non-terminal node representation than terminal nodes as code tokens in terms of CrystalBLEU score for the TLC dataset, about ten times better for Funcom dataset, and about seven times better for the PCSD dataset. The main reason for these improvements is that the vocabulary size of types of non-terminal nodes is significantly less than code tokens. \textbf{We prove that Neural Machine Translation performs significantly better in inferring ASTTrans Representation of AST over inferring Code Tokens from queries for the CAT benchmark.}
\subsection{RQ2. Code Search Application.}
\input{figTabAlgs/tbl_rq2_icse}
The results of RQ2 are shown in Table \ref{asttrans:tbl:rq2}. The augmented embedding for queries and candidates brought a positive effect (Eff.) in MRR for both test sets of four datasets. ASTTrans achieved the best improvement in the TLC dataset for three Java datasets, which has the Average EffectMRR as 2.48\% for four configurations. For a low dimension size of $20$, the performance of GCB and UniXcoder using original (Org.) embedding decreased to 49.71\% for GCB and 50.12\% for UniXcoder. With the augmented embedding, the combined (Com.) code search improved 3.65\% for GCB and 3.47\% for UniXCoder in MRR. With the high embedding size of the original model as $768$, ASTTrans's augmentation improved the MRR as 1.65\% for GCB and 1.16\% for UniXCoder. For CSN, ASTTrans brought a positive effect with 0.07\% of improvement in MRR on average. The augmentation performed best for CSN with dimension size of $20$ and embedding model as UniXcoder. For the Funcom dataset, ASTTrans improved the MRR to 0.12\% on average. Similar to CSN, we achieved higher improvement for UniXcoder.

ASTTrans also improved the accuracy of code search for the Python dataset PCSD with 19028 queries. It positively affected the MRR for both low-dimension and high-dimension sizes of the original embedding and for both SOTA approaches (App). For low dimension size, ASTTrans improved 1.11\% of MRR for GCB and 1.43\% of MRR for UniXcoder. With a high dimension size of 768, while the original models achieved good accuracy of 73.38\% and 76.3\% for GCB and UniXcoder, ASTTrans can still improve the code search up to 0.67\% of improvement. ASTTrans improved by 0.91\% the MRR of code search over the PCSD dataset. \textbf{The Query-to-ASTTrans Representation by Neural Machine Translation can improve code search for GraphCodeBert and UniXcoder with the average EffectMRR as 2.48\%,0.07\%,0.12\% and 0.91\% for four datasets.} 

\subsection{RQ3. Analyzing Factors of ASTTrans.}
\subsubsection{Configuration with Concatenated Embbeding.}
We show the Average EffectMRR of the code search with the vectors of queries and candidates by concatenated embedding at Table \ref{asttrans:tbl:rq3ConcatEmb}. From the results, we show that the effect on four datasets significantly decreased in this configuration. While the TLC dataset and PCSD dataset still have a positive effect in MRR, concatenated embedding from ASTTrans, Funcom, and CSN had negative effects, meaning that the augmented embedding is worse than the original embedding in this setting. \textbf{Our strategy with combined matrix from original similarity matrix and augmented similarity matrix outperformed the ad-hoc strategy with concatenated embedding.}
\input{figTabAlgs/tbl_rq3_concatEmb}

\subsubsection{Varying Combined Weight between Matrix.}
\input{figTabAlgs/fig_rq3_p2}
An advantage of using a combined similarity matrix over concatenated embedding is that we can adjust the combined weight to variate the ratio of the augmented code search to the combined code search. We illustrate this variation by Figure \ref{asttrans:fig:rq3_weight}. We show that with a high weight as close to one, the augmented embedding caused negative impacts on the original model. With the weight up to 0.2, the augmented embedding brings a positive impact.  \textbf{The embedding provided by ASTTrans can positively affect original embedding with the combined weight less than $0.3$.}
\subsubsection{Depth of ASTTrans Representation.}
\input{figTabAlgs/fig_rq3_depth}
The result of the Average EffectMRR over different depths for ASTTrans Representation is shown in Figure \ref{asttrans:fig:rq3_depth}. We changed the depth from $2$ to $9$ for this experiment. The result shows that the depth for best performance in code search varied for each dataset. TLC achieved the highest accuracy at $depth=7$, while PCSD got the best performance in code search with augmented embedding from AST with \textbf{depth=4}. \textbf{In both of datasets, the performance tends to be low with the smallest depth and highest depth. It prove that ASTTrans representation tends to perform best with the middle of depth for AST representation from $depth \in [2,9]$.}
\subsubsection{Cross-datasets Testing for ASTTrans.}
\input{figTabAlgs/tbl_rq3_crossDatasets}
From the result shown in Table \ref{asttrans:tbl:rq3_crossDatasets}, we see that trained models of ASTTrans made positive effect in MRR for nine over 12 settings of cross-dataset training. For cross-datasets code search within Java language, TLC achieved the best code search improvement over the other three datasets. Besides, using the best ASTTrans Representation learning model from the ASTTrans’s model trained on TLC can bring positive EffectMRR for code search with PCSD. \textbf{It shows that ASTTrans can be able to make a positive effect on code search's accuracy with cross-datasets and cross-language testing.}



==> content/ExperimentSetup.tex <==
\section{Experiment Setup}
In the experiment, we attempt to answer the following research questions (RQs):
\begin{enumerate}
    \item RQ1. How superior is query-to-ASTTrans Representation w.r.t query-to-code tokens in NMT?
    \item RQ2. Can a downstream task such as code search benefit from query-to-ASTTrans Representation?
    \item RQ3. Which parameters of query-to-ASTTrans Representation can affect the performance of code search?
\end{enumerate}
In this section, we discuss about the datasets we use, the configurations we set for the experiments, and how we set them up to answer these RQs. 
\subsection{Dataset}
\input{figTabAlgs/tbl_DatasetStat}
We use the CAT benchmark \cite{004_CATBenchmark} with four datasets of code comment at method declaration levels and their corresponding source code as the datasets for training, selecting combination weight $w$ of ASTTrans representation and testing. Different from code search process datasets such as the full version of CodeSearchNet \cite{002_GCB}, information on code comments in the CAT benchmark was normalized by the work of Si et al. \cite{004_CATBenchmark}. There are three Java datasets, including TLCodesum (TLC) (which is the cleaner version of the original TLC dataset proposed in \cite{005_TLC}), Funcom (the cleaner version of \cite{008_Funcom}), CodeSearchNet (CSN) (the cleaner version of \cite{006_CSN}) and one Python dataset named PCSD (the cleaner version of \cite{007_PCSD}). Statistics on four datasets can be shown in Table \ref{asttrans:tbl:dataset}. 
\subsection{Configurations}
\textbf{OpenNMT.} We set up the machine translation model for inferring ASTTrans Representation from the query with the following configurations. We use two sets of neural network layers for training, one as the encoder layer and another as the decoder layer. Each module (encoder/decoder) has two layers, and each layer has 500 hidden units. The gate type to use in each hidden unit is Long Short Term Memory (LSTM). We choose this gate type because LSTM has been proven as an efficient Recurrent Neural Network (RNN) model that can learn and capture the relationship between words in a long textual sequence \cite{003_OpenNMT,027_NMT_google}. We use \textbf{100000} steps for training, with a validating step performed per each \textbf{1000} steps. The check point will be saved for each \textbf{10000} step. In other configurations, we use the default settings from OpenNMT \cite{003_OpenNMT}.

\textbf{fastText.} We use fastText \cite{022_fastText} for text-to-vector conversion using in augmenting query and candidates. fastText \cite{022_fastText} has been proofed as not only the lightweight embedding model but also represents a sequence of text with better accuracy than other textual embedding models such as Doc2Vec \cite{032_Doc2Vec} and TF-IDF \cite{033_TFIDF}, which has been proofed by SE researches \cite{031_fastTextOutperformDoc2Vec}. In our work, we use the augmented dimension size as \textbf{100} and the \textbf{skip-gram} method in fastText for training and generating vectors for augmented embedding.

\textbf{Original Embedding Models.} We use GraphCodeBERT \cite{002_GCB} and UniXCoder \cite{001_UniXcoder} as the SOTA approaches. We used the pre-trained models for Java, and Python developed by GCB and UniXcoder' authors Daja Guo et al. \cite{002_GCB,001_UniXcoder}. We discuss with the SOTA approaches' authors and found out that there are two settings for code search: without fine-tuning and with fine-tuning. The configuration without fine-tuning is called zero-short learning, always performed with much less accuracy than the fine-tuning setting. We also discussed with the SOTA approaches' authors and got confirmation that the accuracy of the two configurations are valid. Thus, we select the better setting, with fine-tuning for our work. We fine-tuned the pre-trained models of GCB and UniXcoder by their proposed dataset CodeSearchNet (CSN) for Java and Python programming  languages. We used the fine-tuned models to generate the embedding for code search of TLC, CSN, Funcom, and PCSD datasets. While the code search for finding the best combination weight of augemntation was done on the validation set of these datasets, our upcoming experiments were run on the testing subset of four datasets (see Table \ref{asttrans:tbl:dataset}.

\textbf{ASTTrans's Augmented Embedding Models.} For the standard configuration that we use in the first two RQs, we trained four query-to-ASTTrans Representation models for four datasets in CAT benchmarks \cite{004_CATBenchmark}. There are two important parameters for ASTTrans. First, we set the depth $k$ of ASTTrans Representation (i.e., the variable $astDepth$ in Listing \ref{asttrans:algm:augmentEmbeddingForCandidates}) as \textbf{the depth size $k=5$}. To come up with this default depth size, we analyze the AST depth, and we found that the average depth of ASTs in the CAT benchmark is \textbf{9}, so we set the default depth as the closest number to the middle of the average depth of ASTs. The second parameter is the weight of combining matrixes of original embedding and augmented embedding. From the code search on the validation subset shown in Table \ref{asttrans:tbl:dataset}, we select the best  combination weight as $w=0.1$. In the analysis experiment in RQ3, we changed these parameters to see how they affect the performance of AStTrans in code search improvement. 

\textbf{Embedding Size of original embedding models and augmented embedding models.} We realize the default dimension of vector generated by GCB and UniXcoder are \textbf{768}, which is quite large compared to embedding size used in other research works in SE such as story point estimation (\cite{034_HeteroSP} - their model required the dimension size as 100) and in general such as Doc2Vec (\cite{032_Doc2Vec} - their model required the dimension size as a range from 100 to 300). Besides, we realize that reduced dimension to SOTA embedding by Principal Component Analysis (PCA) \cite{035_PCA} can bring the improvement on running time as five times faster at dimension size as \textbf{20}. \textbf{So that, we use two dimension sizes for $dim$ as $dim=[20,768]$ for experiments in RQ2 and RQ3.} For the first dimension, we reduce the vectors of the default dimension to a new dimension of 20 using PCA. \textbf{For the augmented embedding, we use the default embedding size suggested by fastText \cite{022_fastText} as 100.}

Both Original Models training and testing and Augmented Models training and testing were trained on a Linux computer with 96 GB of RAM using a Core-i9 processor with 16 cores and a RTX-3080 GPU card with 24GB of RAM. 

\subsection{RQ1.How superior is query-to-ASTTrans Representation w.r.t query-to-code tokens in NMT?}
In this RQ, we want to test whether the NMT model can infer the ASTTrans Representation with higher accuracy than the code tokens given the input as a natural language description of the query. From the CAT benchmark \cite{004_CATBenchmark}, we create four set parallel corpora trained on four datasets. In each set of parallel corpora, we have two parallel corpora with the same source language as textual information of NL queries. The differences between them are the sequences in the target language. While the corpus for query-to-code tokens translation requires the output as source code of candidates, the corpus for query-to-ASTTrans Representation learns the mapping from query to the sequence-based textual representation of candidates' AST at a specific depth like we already mentioned in Definition \ref{asttrans:eq:asttransTextSeq}. 

\textbf{Metrics for RQ1's evaluation.} Similar to other NMT problems such as natural language translation \cite{027_NMT_google}, the quality of a machine translation system is evaluated by the similarity between the expected result from the parallel corpus and the predicted result as a sequence of tokens suggested by the NMT model. While the BLEU score \cite{036_BLEU} has been used frequently for evaluating the performance of NMT in Natural Language Processing. However, in SE, the BLEU score has been proven that reveal drawbacks while performing on source code dataset due to the repetitiveness of the source code \cite{009_CrystalBLEU} and the mismatch of BLEU's results compared to human judgment \cite{037_METEOR_Study}. Michael Pradel et al. \cite{009_CrystalBLEU} proposed an approach for filtering repetitive n-grams for calculating textual similarity in source code and defined a new metric named Crystal-BLEU-4 (number four stands for four-gram cumulatively, the default configuration of Crystal-BLEU). Besides, on the NLP-based textual similarity comparison metrics list, Roy et al. \cite{037_METEOR_Study} shows that Meteor \cite{010_Meteor} score can perform better than BLEU score by an evaluation based on human judgment. With the fact that both \textbf{Crystal-BLEU-4} \cite{009_CrystalBLEU} and \textbf{Meteor} \cite{010_Meteor} has been proven effective in SE tasks, we choose these metrics for evaluating the performance of NMT for RQ1.

\subsection{RQ2. Can a downstream task such as code search benefit from query-to-ASTTrans Representation?}
In this RQ, we evaluate the effect of the augmented embedding provided by ASTTrans in improving the original embedding models, i.e., SOTA approaches as GCB and UniXcoder. Next, we discuss about the metrics that are used for evaluation in code search and our defined metrics for measuring how ASTTrans can increase/decrease the accuracy of SOTA approaches.
\subsubsection{Metrics for Evaluating Code Search.}

\textbf{Top-K accuracy.} We use the same definition of Top-K accuracy used in SOTA approaches \cite{001_UniXcoder,002_GCB}. Given a case of code search with a query and a list of candidates as the code search result of that query, the top-K accuracy on a set of cases is the ratio of the cases that the correct candidate appears within the first K candidates of the returned list over the number of cases. We will use the top-K accuracy in the Ablation Study section.

\textbf{Mean Reciprocal Rank (MRR).} Given a set of cases of code search $C$, the MRR of the code search over this set is calculated by Formula \ref{asttrans:eq:definitionMRR}:
\begin{equation}
    MRR(C)=\frac{1}{|C|}*\sum_{c \in C}^{}\frac{1}{rank_{c}}
    \label{asttrans:eq:definitionMRR}
\end{equation}
In this formula, \textbf{$rank_{c}$ }is the index of the correct candidate in the returned list of candidates for a code search case $c$. In our work, the MRR score on a code search case $C$ will differ by the original/augmented embedding models and their dimension size. 
\subsubsection{Metrics for Evaluating the Effect of ASTTrans to Original Models.}

\textbf{Effect in MRR.} The effect in MRR over code search on set $C$ of cases by ASTTrans embedding $a$ to original embedding model $o$ with original embedding size $d$, is calculated by Formula \ref{asttrans:eq:definitionEffectMRR}:
\begin{equation}
    EffectMRR(C,a,o,d)=MRR_{com}(C,a,o,d)-MRR_{org}(C,a,o,d)
    \label{asttrans:eq:definitionEffectMRR}
\end{equation}
In this Formula, $MRR_{org}$ is the MRR returned by original code search, and $MRR_{com}$ is the MRR returned by code search with the combined matrix from original cosine similarity matrix and augmented cosine similarity matrix for a specific set of candidates, original model, and augmented model. If the result of this metric is positive, it means the augmented embedding improved the accuracy of the original embedding model by MRR. Since we run the default experiment of 2 SOTA original embedding models with two different original embedding sizes, we defined the metric Average of Effect in MRR, called A, by the $Average_{EffectMRR}(C)$ as the average of EffectMRR over a set of cases $C$ with four configurations: $o \in [GCB,UniXcoder]$ and $d \in [20,768]$.

\subsection{RQ3. Which parameters of query-to-ASTTrans Representation can affect the performance of code search?}
In this RQ, we attempt to validate the performance of ASTTrans in improving code search for SOTA embedding models with different settings. We select the following parameters.

\textbf{Concatenating Vectors versus Combining Matrices.} In the default configuration, we create two matrices representing the similarities between the original embedding model and augmented embedding models between queries and candidates (see Figure \ref{asttrans:fig:overview}). There is another strategy to combine the embedding of ASTTrans Representation by concatenating elements of embedding in ASTTrans to the original embedding model and performing code search with the combined embedding. Given a query $A_{1}$, the original embedding $\overrightarrow{n}=[n_{1},n_{2}]$ and the augmented embedding $\overrightarrow{n^{'}}=[n^{'}_{1},n^{'}_{2}]$, the concatenated vector for code search is $\overrightarrow{n^{''}}=[n_{1},n_{2},n^{'}_{1},n^{'}_{2}]$. In the first part of this RQ, we change the strategy of augmentation to use the combined vector for code search and evaluate the performance of code search with this strategy.

\textbf{Combined weight between matrices.}  By default, we select the weight of the similarity matrix by augmented embedding $w$  as 0.1. In the second part of this RQ, we run the code search with different weights from 0.2 to 1 with the seed as 0.1 to analyze the performance of ASTTrans with different combined weights.

\textbf{Depth of ASTTrans Representation.} While the default depth of ASTTrans Representation is $depth=5$, we wondered how well a sequence of non-terminal nodes with different depths from the root can perform in improving code search. In our assumption, the representation of a non-terminal node at a lower depth might be easier for NMT to learn the information, but it has the risk of not giving enough information for code search. For example, the ASTTrans Representation at $depth=0$ returns the root node for every candidate, meaning that representation cannot differentiate candidates for code search. Since the non-terminal nodes at $depth<2$ are too abstract, we select the range of $depth \in [2,9]$ to evaluate the code search process.

\textbf{Cross-datasets training.} In this part of RQ3, we use the trained model from one dataset to predict the ASTTrans Representation of candidates in the different datasets to compare how it performs in code search improvement. Since we have four datasets, there are  12 different configurations for code search.




% \subsection{RQ2.}
% \subsection{RQ3.}
% \subsection{Dataset}
% \input{figTabAlgs/tbl_DatasetStat}
% \subsection{Configurations}
% \subsubsection{Original Embedding}
% \subsubsection{Neural Machine Translation}




==> content/Introduction_arxiv.tex <==
\section{Introduction}
% OpenNMT Neural Machine Translation
Neural Machine Translation (NMT) \cite{027_NMT_google} is a deep learning-based approach for inferring textual sequences between different Natural Languages (NL). Since NMT has been applied successfully in NL translation in Natural Language Processing (NLP), the advantages of NMT have been used in various problems of Software Engineering (SE) \cite{014_DeepTyper,020_NMT_CodeChange}. Recent work shows that NMT model can outperform the current-trend translation approach CodeT5 \cite{024_CodeT5} in explaining bugs from code changes \cite{021_NMT_BugExplain}. NMT's advantages are learning relationships on the textual sequence as input by Long-Short-Term-Memory (LSTM) and connecting information between the source language and target language by attention model \cite{027_NMT_google}. The basic idea of applying NMT to SE is to define the source and target languages in the problems that NMT is intended to solve. For example, with bug explanation, the source language is the sequence of code tokens as source code, and the target language is the bug description \cite{021_NMT_BugExplain}. With type inference, the source language is incomplete code that lacks information about types, and the target language is complete code with types \cite{014_DeepTyper}.

Code Generation from NL artifacts is a research problem that has gained more interest in the last decade \cite{025_SPoC,002_GCB}. Since this problem can be formalized as a language translation problem considering NL artifacts as the source language and the code tokens as the target language, NMT can be a means of solving this problem. From types of the NL artifacts as input for NMT, the pseudocode of code tokens has been studied in many works \cite{025_SPoC}. Pseudocode, often written in the form of informal natural language, is used to help software developers write algorithms in textual description \cite{029_pseudocodeExample}. To the best of our knowledge, the projects of Kulal et al. \cite{025_SPoC} and Zhong et al. \cite{026_Scaffold} are the latest projects that have applied NMT for pseudocode-to-code translation. They apply NMT for solving pseudocode-to-code translation and optimize the output of NMT as translated code pieces by different modules of error localization \cite{025_SPoC} and program analysis \cite{026_Scaffold}. 

Although NMT has been proven effective in pseudocode-to-code translation \cite{025_SPoC,026_Scaffold}, applying NMT on practical datasets of real-world NL queries and code snippets might fail due to two reasons. First, in real-world benchmarks like the CAT benchmark \cite{004_CATBenchmark} NL queries usually have significantly fewer words than the number of tokens in their corresponding source code. NL query is a type of code documentation used to explain how its source code works with short descriptions as summarization. The lack of mapping between each Line of Code (LOC) to its description in code snippets of CAT benchmark might reduce the quality of NMT translation models on datasets in CAT benchmark compared to pseudocode-to-code translation. Second, NMT usually outputs incomplete code snippets that require error localization and fixing \cite{025_SPoC}. It considers the output a sequence of code tokens instead of an Abstract Syntax Tree (AST) representation. Unlike translation, code retrieval by code search \cite{001_UniXcoder} can return complete code. 

In this work, we analyze the performance of NMT on learning specific information about the source code by AST's subset of non-terminal nodes, compared to learning from NL query to code tokens. We propose ASTTrans, an NMT translation engine trained using OpenNMT toolkit \cite{003_OpenNMT} to learn the mapping from documentation to our tailored representation of an AST by non-terminal nodes. Then, we build a new code search approach that integrates ASTTrans to the state-of-the-art (SOTA) code search process embedding models \cite{001_UniXcoder,002_GCB}. Overall, our contributions are as follows:
\begin{enumerate}     
\item We analyze and demonstrate NMT in learning our tailored representation of AST compared to learning the sequence of code tokens.
\item We build a query-to-ASTTrans Representation model and integrate its output to improve the accuracy of the SOTA code search models GraphCodeBERT \cite{002_GCB} and UniXcoder \cite{001_UniXcoder} and achieve up to 3.08\% MRR improvement on TLC dataset and 1.06\% on average on all datasets of CAT benchmark.
\item We analyze how the parameters of ASTTrans can impact the performance in code search.
\item We conduct a case study to investigate the reasons when ASTTrans can or cannot improve the code search for SOTA models.
\end{enumerate}
The rest of this paper is organized as follows. In section 2, Motivation Example, we introduce an example of a query/ candidate for a code search problem. Section 3 provides background information, summarizing the approaches provided in existing embedding tools GraphCodeBERT\cite{002_GCB} and UniXcoder \cite{001_UniXcoder}. Section 4 shows definitions related to our proposed representation  of AST. Section 5 describes in detail our approach to integrating ASTTrans into the original code search process by SOTA approaches. Section 6 mentions our experiments, including configurations, metrics, and results of our proposed research questions. In section 7, we conduct a case study about when ASTTrans can/cannot improve original models. The remaining sections are Related Work, Threats to Validity, and Conclusion. 

==> content/refs.tex <==
@misc{001_UniXcoder,
  doi = {10.48550/ARXIV.2203.03850},
  
  url = {https://arxiv.org/abs/2203.03850},
  
  author = {Guo, Daya and Lu, Shuai and Duan, Nan and Wang, Yanlin and Zhou, Ming and Yin, Jian},
  
  keywords = {Computation and Language (cs.CL), Programming Languages (cs.PL), Software Engineering (cs.SE), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {UniXcoder: Unified Cross-Modal Pre-training for Code Representation},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{002_GCB,
  author    = {Daya Guo and
               Shuo Ren and
               Shuai Lu and
               Zhangyin Feng and
               Duyu Tang and
               Shujie Liu and
               Long Zhou and
               Nan Duan and
               Alexey Svyatkovskiy and
               Shengyu Fu and
               Michele Tufano and
               Shao Kun Deng and
               Colin B. Clement and
               Dawn Drain and
               Neel Sundaresan and
               Jian Yin and
               Daxin Jiang and
               Ming Zhou},
  title     = {GraphCodeBERT: Pre-training Code Representations with Data Flow},
  journal   = {CoRR},
  volume    = {abs/2009.08366},
  year      = {2020},
  url       = {https://arxiv.org/abs/2009.08366},
  eprinttype = {arXiv},
  eprint    = {2009.08366},
  timestamp = {Tue, 13 Oct 2020 10:46:35 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2009-08366.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{003_OpenNMT,
    title = "OpenNMT: Open-Source Toolkit for Neural Machine Translation",
    author = "Klein, Guillaume  and
      Kim, Yoon  and
      Deng, Yuntian  and
      Senellart, Jean  and
      Rush, Alexander",
    booktitle = "Proceedings of ACL 2017, System Demonstrations",
    month = jul,
    year = "2017",
    address = "Vancouver, Canada",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P17-4012",
    pages = "67--72",
}

@inproceedings{004_CATBenchmark,
author = {Shi, Lin and Mu, Fangwen and Chen, Xiao and Wang, Song and Wang, Junjie and Yang, Ye and Li, Ge and Xia, Xin and Wang, Qing},
title = {Are We Building on the Rock? On the Importance of Data Preprocessing for Code Summarization},
year = {2022},
isbn = {9781450394130},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3540250.3549145},
doi = {10.1145/3540250.3549145},
abstract = {Code summarization, the task of generating useful comments given the code, has long been of interest. Most of the existing code summarization models are trained and validated on widely-used code comment benchmark datasets. However, little is known about the quality of the benchmark datasets built from real-world projects. Are the benchmark datasets as good as expected? To bridge the gap, we conduct a systematic research to assess and improve the quality of four benchmark datasets widely used for code summarization tasks. First, we propose an automated code-comment cleaning tool that can accurately detect noisy data caused by inappropriate data preprocessing operations from existing benchmark datasets. Then, we apply the tool to further assess the data quality of the four benchmark datasets, based on the detected noises. Finally, we conduct comparative experiments to investigate the impact of noisy data on the performance of code summarization models. The results show that these data preprocessing noises widely exist in all four benchmark datasets, and removing these noisy data leads to a significant improvement on the performance of code summarization. We believe that the findings and insights will enable a better understanding of data quality in code summarization tasks, and pave the way for relevant research and practice.},
booktitle = {Proceedings of the 30th ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
pages = {107–119},
numpages = {13},
keywords = {Code Summarization, Empirical Study, Data Quality},
location = {Singapore, Singapore},
series = {ESEC/FSE 2022}
}

@inproceedings{005_TLC,
author = {Hu, Xing and Li, Ge and Xia, Xin and Lo, David and Lu, Shuai and Jin, Zhi},
title = {Summarizing Source Code with Transferred API Knowledge},
year = {2018},
isbn = {9780999241127},
publisher = {AAAI Press},
abstract = {Code summarization, aiming to generate succinct natural language description of source code, is extremely useful for code search and code comprehension. It has played an important role in software maintenance and evolution. Previous approaches generate summaries by retrieving summaries from similar code snippets. However, these approaches heavily rely on whether similar code snippets can be retrieved, how similar the snippets are, and fail to capture the API knowledge in the source code, which carries vital information about the functionality of the source code. In this paper, we propose a novel approach, named TL-CodeSum, which successfully uses API knowledge learned in a different but related task to code summarization. Experiments on large-scale real-world industry Java projects indicate that our approach is effective and outperforms the state-of-the-art in code summarization.},
booktitle = {Proceedings of the 27th International Joint Conference on Artificial Intelligence},
pages = {2269–2275},
numpages = {7},
location = {Stockholm, Sweden},
series = {IJCAI'18}
}

@misc{006_CSN,
  doi = {10.48550/ARXIV.1909.09436},
  
  url = {https://arxiv.org/abs/1909.09436},
  
  author = {Husain, Hamel and Wu, Ho-Hsiang and Gazit, Tiferet and Allamanis, Miltiadis and Brockschmidt, Marc},
  
  keywords = {Machine Learning (cs.LG), Information Retrieval (cs.IR), Software Engineering (cs.SE), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {CodeSearchNet Challenge: Evaluating the State of Semantic Code Search},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{007_PCSD,
author = {Wan, Yao and Zhao, Zhou and Yang, Min and Xu, Guandong and Ying, Haochao and Wu, Jian and Yu, Philip S.},
title = {Improving Automatic Source Code Summarization via Deep Reinforcement Learning},
year = {2018},
isbn = {9781450359375},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3238147.3238206},
doi = {10.1145/3238147.3238206},
abstract = {Code summarization provides a high level natural language description of the function performed by code, as it can benefit the software maintenance, code categorization and retrieval. To the best of our knowledge, most state-of-the-art approaches follow an encoder-decoder framework which encodes the code into a hidden space and then decode it into natural language space, suffering from two major drawbacks: a) Their encoders only consider the sequential content of code, ignoring the tree structure which is also critical for the task of code summarization; b) Their decoders are typically trained to predict the next word by maximizing the likelihood of next ground-truth word with previous ground-truth word given. However, it is expected to generate the entire sequence from scratch at test time. This discrepancy can cause an exposure bias issue, making the learnt decoder suboptimal. In this paper, we incorporate an abstract syntax tree structure as well as sequential content of code snippets into a deep reinforcement learning framework (i.e., actor-critic network). The actor network provides the confidence of predicting the next word according to current state. On the other hand, the critic network evaluates the reward value of all possible extensions of the current state and can provide global guidance for explorations. We employ an advantage reward composed of BLEU metric to train both networks. Comprehensive experiments on a real-world dataset show the effectiveness of our proposed model when compared with some state-of-the-art methods.},
booktitle = {Proceedings of the 33rd ACM/IEEE International Conference on Automated Software Engineering},
pages = {397–407},
numpages = {11},
keywords = {deep learning, reinforcement learning, Code summarization, comment generation},
location = {Montpellier, France},
series = {ASE '18}
}

@inproceedings{008_Funcom,
    title = "Code to Comment Translation: A Comparative Study on Model Effectiveness {\&} Errors",
    author = "Mahmud, Junayed  and
      Faisal, Fahim  and
      Arnob, Raihan Islam  and
      Anastasopoulos, Antonios  and
      Moran, Kevin",
    booktitle = "Proceedings of the 1st Workshop on Natural Language Processing for Programming (NLP4Prog 2021)",
    month = aug,
    year = "2021",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2021.nlp4prog-1.1",
    doi = "10.18653/v1/2021.nlp4prog-1.1",
    pages = "1--16",
    abstract = "Automated source code summarization is a popular software engineering research topic wherein machine translation models are employed to {``}translate{''} code snippets into relevant natural language descriptions. Most evaluations of such models are conducted using automatic reference-based metrics. However, given the relatively large semantic gap between programming languages and natural language, we argue that this line of research would benefit from a qualitative investigation into the various error modes of current state-of-the-art models. Therefore, in this work, we perform both a quantitative and qualitative comparison of three recently proposed source code summarization models. In our quantitative evaluation, we compare the models based on the smoothed BLEU-4, METEOR, and ROUGE-L machine translation metrics, and in our qualitative evaluation, we perform a manual open-coding of the most common errors committed by the models when compared to ground truth captions. Our investigation reveals new insights into the relationship between metric-based performance and model prediction errors grounded in an error taxonomy that can be used to drive future research efforts.",
}
@inproceedings{009_CrystalBLEU,
author = {Eghbali, Aryaz and Pradel, Michael},
title = {CrystalBLEU: Precisely and Efficiently Measuring the Similarity of Code},
year = {2023},
isbn = {9781450394758},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3551349.3556903},
doi = {10.1145/3551349.3556903},
abstract = {Recent years have brought a surge of work on predicting pieces of source code, e.g., for code completion, code migration, program repair, or translating natural language into code. All this work faces the challenge of evaluating the quality of a prediction w.r.t. some oracle, typically in the form of a reference solution. A common evaluation metric is the BLEU score, an n-gram-based metric originally proposed for evaluating natural language translation, but adopted in software engineering because it can be easily computed on any programming language and enables automated evaluation at scale. However, a key difference between natural and programming languages is that in the latter, completely unrelated pieces of code may have many common n-grams simply because of the syntactic verbosity and coding conventions of programming languages. We observe that these trivially shared n-grams hamper the ability of the metric to distinguish between truly similar code examples and code examples that are merely written in the same language. This paper presents CrystalBLEU, an evaluation metric based on BLEU, that allows for precisely and efficiently measuring the similarity of code. Our metric preserves the desirable properties of BLEU, such as being language-agnostic, able to handle incomplete or partially incorrect code, and efficient, while reducing the noise caused by trivially shared n-grams. We evaluate CrystalBLEU on two datasets from prior work and on a new, labeled dataset of semantically equivalent programs. Our results show that CrystalBLEU can distinguish similar from dissimilar code examples 1.9–4.5 times more effectively, when compared to the original BLEU score and a previously proposed variant of BLEU for code.},
booktitle = {Proceedings of the 37th IEEE/ACM International Conference on Automated Software Engineering},
articleno = {28},
numpages = {12},
keywords = {Evaluation, Metric, BLEU},
location = {Rochester, MI, USA},
series = {ASE '22}
}
@InProceedings{010_Meteor,
  author    = {Michael Denkowski and Alon Lavie},
  title     = {Meteor Universal: Language Specific Translation Evaluation for Any Target Language},
  booktitle = {Proceedings of the EACL 2014 Workshop on Statistical Machine Translation},
  year      = {2014},
}
@inproceedings{10.3115/1073083.1073135,
author = {Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
title = {BLEU: A Method for Automatic Evaluation of Machine Translation},
year = {2002},
publisher = {Association for Computational Linguistics},
address = {USA},
url = {https://doi.org/10.3115/1073083.1073135},
doi = {10.3115/1073083.1073135},
abstract = {Human evaluations of machine translation are extensive but expensive. Human evaluations can take months to finish and involve human labor that can not be reused. We propose a method of automatic machine translation evaluation that is quick, inexpensive, and language-independent, that correlates highly with human evaluation, and that has little marginal cost per run. We present this method as an automated understudy to skilled human judges which substitutes for them when there is need for quick or frequent evaluations.},
booktitle = {Proceedings of the 40th Annual Meeting on Association for Computational Linguistics},
pages = {311–318},
numpages = {8},
location = {Philadelphia, Pennsylvania},
series = {ACL '02}
}
@inproceedings{012_ROUGE,
    title = "{ROUGE}: A Package for Automatic Evaluation of Summaries",
    author = "Lin, Chin-Yew",
    booktitle = "Text Summarization Branches Out",
    month = jul,
    year = "2004",
    address = "Barcelona, Spain",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/W04-1013",
    pages = "74--81",
}
@inproceedings{013_ROUGE_DRAWBACKS,
    title = "The limits of automatic summarisation according to {ROUGE}",
    author = "Schluter, Natalie",
    booktitle = "Proceedings of the 15th Conference of the {E}uropean Chapter of the Association for Computational Linguistics: Volume 2, Short Papers",
    month = apr,
    year = "2017",
    address = "Valencia, Spain",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/E17-2007",
    pages = "41--45",
    abstract = "This paper discusses some central caveats of summarisation, incurred in the use of the ROUGE metric for evaluation, with respect to optimal solutions. The task is NP-hard, of which we give the first proof. Still, as we show empirically for three central benchmark datasets for the task, greedy algorithms empirically seem to perform optimally according to the metric. Additionally, overall quality assurance is problematic: there is no natural upper bound on the quality of summarisation systems, and even humans are excluded from performing optimal summarisation.",
}
@inproceedings{014_DeepTyper,
author = {Hellendoorn, Vincent J. and Bird, Christian and Barr, Earl T. and Allamanis, Miltiadis},
title = {Deep Learning Type Inference},
year = {2018},
isbn = {9781450355735},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3236024.3236051},
doi = {10.1145/3236024.3236051},
abstract = {Dynamically typed languages such as JavaScript and Python are increasingly popular, yet static typing has not been totally eclipsed: Python now supports type annotations and languages like TypeScript offer a middle-ground for JavaScript: a strict superset of JavaScript, to which it transpiles, coupled with a type system that permits partially typed programs. However, static typing has a cost: adding annotations, reading the added syntax, and wrestling with the type system to fix type errors. Type inference can ease the transition to more statically typed code and unlock the benefits of richer compile-time information, but is limited in languages like JavaScript as it cannot soundly handle duck-typing or runtime evaluation via eval. We propose DeepTyper, a deep learning model that understands which types naturally occur in certain contexts and relations and can provide type suggestions, which can often be verified by the type checker, even if it could not infer the type initially. DeepTyper, leverages an automatically aligned corpus of tokens and types to accurately predict thousands of variable and function type annotations. Furthermore, we demonstrate that context is key in accurately assigning these types and introduce a technique to reduce overfitting on local cues while highlighting the need for further improvements. Finally, we show that our model can interact with a compiler to provide more than 4,000 additional type annotations with over 95% precision that could not be inferred without the aid of DeepTyper.},
booktitle = {Proceedings of the 2018 26th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
pages = {152–162},
numpages = {11},
keywords = {Type Inference, Naturalness, Deep Learning},
location = {Lake Buena Vista, FL, USA},
series = {ESEC/FSE 2018}
}

@inproceedings{015_StatGen,
author = {Nguyen, Hoan Anh and Phan, Hung Dang and Khairunnesa, Samantha Syeda and Nguyen, Son and Yadavally, Aashish and Wang, Shaohua and Rajan, Hridesh and Nguyen, Tien},
title = {A Hybrid Approach for Inference between Behavioral Exception API Documentation and Implementations, and Its Applications},
year = {2023},
isbn = {9781450394758},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3551349.3560434},
doi = {10.1145/3551349.3560434},
abstract = {Automatically producing behavioral exception (BE) API documentation helps developers correctly use the libraries. The state-of-the-art approaches are either rule-based, which is too restrictive in its applicability, or deep learning (DL)-based, which requires large training dataset. To address that, we propose StatGen, a novel hybrid approach between statistical machine translation (SMT) and tree-structured translation to generate the BE documentation for any code and vice versa. We consider the documentation and source code of an API method as the two abstraction levels of the same intent. StatGen is specifically designed for this two-way inference, and takes advantage of their structures for higher accuracy. We conducted several experiments to evaluate StatGen. We show that it achieves high precision (75% and 75%), and recall (81% and 84%), in inferring BE documentation from source code and vice versa. StatGen achieves higher precision, recall, and BLEU score than the state-of-the-art, DL-based baseline models. We show StatGen’s usefulness in two applications. First, we use it to generate the BE documentation for Apache APIs that lack of documentation by learning from the documentation of the equivalent APIs in JDK. 44% of the generated documentation were rated as useful and 42% as somewhat useful. In the second application, we use StatGen to detect the inconsistency between the BE documentation and corresponding implementations of several JDK8 packages.},
booktitle = {Proceedings of the 37th IEEE/ACM International Conference on Automated Software Engineering},
articleno = {2},
numpages = {13},
keywords = {Inference between Documentation and Code, Behavioral Exception Specification, Hybrid Machine Translation},
location = {Rochester, MI, USA},
series = {ASE '22}
}

@inproceedings{016_StatType,
author = {Phan, Hung and Nguyen, Hoan Anh and Tran, Ngoc M. and Truong, Linh H. and Nguyen, Anh Tuan and Nguyen, Tien N.},
title = {Statistical Learning of API Fully Qualified Names in Code Snippets of Online Forums},
year = {2018},
isbn = {9781450356381},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3180155.3180230},
doi = {10.1145/3180155.3180230},
abstract = {Software developers often make use of the online forums such as StackOverflow (SO) to learn how to use software libraries and their APIs. However, the code snippets in such a forum often contain undeclared, ambiguous, or largely unqualified external references. Such declaration ambiguity and external reference ambiguity present challenges for developers in learning to correctly use the APIs. In this paper, we propose StatType, a statistical approach to resolve the fully qualified names (FQNs) for the API elements in such code snippets. Unlike existing approaches that are based on heuristics, StatType has two well-integrated factors. We first learn from a large training code corpus the FQNs that often co-occur. Then, to derive the FQN for an API name in a code snippet, we use that knowledge and also leverage the context consisting of neighboring API names. To realize those factors, we treat the problem as statistical machine translation from source code with partially qualified names to source code with FQNs of the APIs. Our empirical evaluation on real-world code and StackOverflow posts shows that StatType achieves very high accuracy with 97.6% precision and 96.7% recall, which is 16.5% relatively higher than the state-of-the-art approach.},
booktitle = {Proceedings of the 40th International Conference on Software Engineering},
pages = {632–642},
numpages = {11},
keywords = {statistical machine translation, partial program analysis, naturalness, type inference, big code, type resolution, type annotations},
location = {Gothenburg, Sweden},
series = {ICSE '18}
}

@inproceedings{017_SMT_CodeMigration,
author = {Nguyen, Anh Tuan and Nguyen, Tung Thanh and Nguyen, Tien N.},
title = {Migrating Code with Statistical Machine Translation},
year = {2014},
isbn = {9781450327688},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/2591062.2591072},
doi = {10.1145/2591062.2591072},
abstract = {In the era of mobile computing, developers often need to migrate code written for one platform in a programming language to another language for a different platform, e.g., from Java for Android to C# for Windows Phone. The migration process is often performed manually or semi-automatically, in which developers are required to manually define translation rules and API mappings. This paper presents semSMT, an automatic tool to migrate code written in Java to C#. semSMT utilizes statistical machine translation to automatically infer translation rules from existing migrated code, thus, requires no manual defining of rules. The video demonstration on semSMT can be found on YouTube at http://www.youtube.com/watch?v=aRSnl5-7vNo.},
booktitle = {Companion Proceedings of the 36th International Conference on Software Engineering},
pages = {544–547},
numpages = {4},
keywords = {Language Migration, Statistical Machine Translation},
location = {Hyderabad, India},
series = {ICSE Companion 2014}
}

@article{018_NMT_SoftwareLocalization,
  title={Domain-specific machine translation with recurrent neural network for software localization},
  author={Wang, Xu and Chen, Chunyang and Xing, Zhenchang},
  journal={Empirical Software Engineering},
  volume={24},
  pages={3514--3545},
  year={2019},
  publisher={Springer}
}
@misc{019_NMT_Test,
  doi = {10.48550/ARXIV.1910.02688},
  
  url = {https://arxiv.org/abs/1910.02688},
  
  author = {Sun, Zeyu and Zhang, Jie M. and Harman, Mark and Papadakis, Mike and Zhang, Lu},
  
  keywords = {Software Engineering (cs.SE), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Automatic Testing and Improvement of Machine Translation},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@inproceedings{020_NMT_CodeChange,
author = {Tufano, Michele and Pantiuchina, Jevgenija and Watson, Cody and Bavota, Gabriele and Poshyvanyk, Denys},
title = {On Learning Meaningful Code Changes via Neural Machine Translation},
year = {2019},
publisher = {IEEE Press},
url = {https://doi.org/10.1109/ICSE.2019.00021},
doi = {10.1109/ICSE.2019.00021},
abstract = {Recent years have seen the rise of Deep Learning (DL) techniques applied to source code. Researchers have exploited DL to automate several development and maintenance tasks, such as writing commit messages, generating comments and detecting vulnerabilities among others. One of the long lasting dreams of applying DL to source code is the possibility to automate non-trivial coding activities. While some steps in this direction have been taken (e.g., learning how to fix bugs), there is still a glaring lack of empirical evidence on the types of code changes that can be learned and automatically applied by DL.Our goal is to make this first important step by quantitatively and qualitatively investigating the ability of a Neural Machine Translation (NMT) model to learn how to automatically apply code changes implemented by developers during pull requests. We train and experiment with the NMT model on a set of 236k pairs of code components before and after the implementation of the changes provided in the pull requests. We show that, when applied in a narrow enough context (i.e., small/medium-sized pairs of methods before/after the pull request changes), NMT can automatically replicate the changes implemented by developers during pull requests in up to 36% of the cases. Moreover, our qualitative analysis shows that the model is capable of learning and replicating a wide variety of meaningful code changes, especially refactorings and bug-fixing activities. Our results pave the way for novel research in the area of DL on code, such as the automatic learning and applications of refactoring.},
booktitle = {Proceedings of the 41st International Conference on Software Engineering},
pages = {25–36},
numpages = {12},
keywords = {neural-machine translation, empirical study},
location = {Montreal, Quebec, Canada},
series = {ICSE '19}
}
@misc{021_NMT_BugExplain,
  doi = {10.48550/ARXIV.2212.04584},
  
  url = {https://arxiv.org/abs/2212.04584},
  
  author = {Mahbub, Parvez and Shuvo, Ohiduzzaman and Rahman, Mohammad Masudur},
  
  keywords = {Software Engineering (cs.SE), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Explaining Software Bugs Leveraging Code Structures in Neural Machine Translation},
  
  publisher = {arXiv},
  
  year = {2022},
  
  copyright = {Creative Commons Attribution Non Commercial Share Alike 4.0 International}
}
@article{022_fastText,
  title={Enriching Word Vectors with Subword Information},
  author={Bojanowski, Piotr and Grave, Edouard and Joulin, Armand and Mikolov, Tomas},
  journal={Transactions of the Association for Computational Linguistics},
  volume={5},
  year={2017},
  issn={2307-387X},
  pages={135--146}
}
@misc{023_treesitter,
  title = {{Article on treesitter}},
  howpublished = {\url{https://tinyurl.com/y2a86znt}},
  note = {{Accessed: 2022-6-20}},
}

@inproceedings{
    024_CodeT5,
    title={CodeT5: Identifier-aware Unified Pre-trained Encoder-Decoder Models for Code Understanding and Generation}, 
    author={Yue, Wang and Weishi, Wang and Shafiq, Joty and Steven, C.H., Hoi},
    booktitle={Proceedings of the 2021 Conference on Empirical Methods in Natural Language Processing, EMNLP 2021},
    year={2021},
}
@misc{025_SPoC,
  doi = {10.48550/ARXIV.1906.04908},
  
  url = {https://arxiv.org/abs/1906.04908},
  
  author = {Kulal, Sumith and Pasupat, Panupong and Chandra, Kartik and Lee, Mina and Padon, Oded and Aiken, Alex and Liang, Percy},
  
  keywords = {Machine Learning (cs.LG), Computation and Language (cs.CL), Programming Languages (cs.PL), Machine Learning (stat.ML), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {SPoC: Search-based Pseudocode to Code},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{026_Scaffold,
  author    = {Ruiqi Zhong and
               Mitchell Stern and
               Dan Klein},
  title     = {Semantic Scaffolds for Pseudocode-to-Code Generation},
  journal   = {CoRR},
  volume    = {abs/2005.05927},
  year      = {2020},
  url       = {https://arxiv.org/abs/2005.05927},
  eprinttype = {arXiv},
  eprint    = {2005.05927},
  timestamp = {Thu, 14 May 2020 16:56:02 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-2005-05927.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{027_NMT_google,
  author    = {Yonghui Wu and
               Mike Schuster and
               Zhifeng Chen and
               Quoc V. Le and
               Mohammad Norouzi and
               Wolfgang Macherey and
               Maxim Krikun and
               Yuan Cao and
               Qin Gao and
               Klaus Macherey and
               Jeff Klingner and
               Apurva Shah and
               Melvin Johnson and
               Xiaobing Liu and
               Lukasz Kaiser and
               Stephan Gouws and
               Yoshikiyo Kato and
               Taku Kudo and
               Hideto Kazawa and
               Keith Stevens and
               George Kurian and
               Nishant Patil and
               Wei Wang and
               Cliff Young and
               Jason Smith and
               Jason Riesa and
               Alex Rudnick and
               Oriol Vinyals and
               Greg Corrado and
               Macduff Hughes and
               Jeffrey Dean},
  title     = {Google's Neural Machine Translation System: Bridging the Gap between
               Human and Machine Translation},
  journal   = {CoRR},
  volume    = {abs/1609.08144},
  year      = {2016},
  url       = {http://arxiv.org/abs/1609.08144},
  eprinttype = {arXiv},
  eprint    = {1609.08144},
  timestamp = {Thu, 14 Jan 2021 12:12:19 +0100},
  biburl    = {https://dblp.org/rec/journals/corr/WuSCLNMKCGMKSJL16.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{028_AnalysisPretrainedModelGCB,
author = {Wan, Yao and Zhao, Wei and Zhang, Hongyu and Sui, Yulei and Xu, Guandong and Jin, Hai},
title = {What Do They Capture? A Structural Analysis of Pre-Trained Language Models for Source Code},
year = {2022},
isbn = {9781450392211},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3510003.3510050},
doi = {10.1145/3510003.3510050},
abstract = {Recently, many pre-trained language models for source code have been proposed to model the context of code and serve as a basis for downstream code intelligence tasks such as code completion, code search, and code summarization. These models leverage masked pre-training and Transformer and have achieved promising results. However, currently there is still little progress regarding interpretability of existing pre-trained code models. It is not clear why these models work and what feature correlations they can capture. In this paper, we conduct a thorough structural analysis aiming to provide an interpretation of pre-trained language models for source code (e.g., CodeBERT, and GraphCodeBERT) from three distinctive perspectives: (1) attention analysis, (2) probing on the word embedding, and (3) syntax tree induction. Through comprehensive analysis, this paper reveals several insightful findings that may inspire future studies: (1) Attention aligns strongly with the syntax structure of code. (2) Pre-training language models of code can preserve the syntax structure of code in the intermediate representations of each Transformer layer. (3) The pre-trained models of code have the ability of inducing syntax trees of code. Theses findings suggest that it may be helpful to incorporate the syntax structure of code into the process of pre-training for better code representations.},
booktitle = {Proceedings of the 44th International Conference on Software Engineering},
pages = {2377–2388},
numpages = {12},
keywords = {pre-trained language model, probing, attention analysis, deep learning, syntax tree induction, code representation},
location = {Pittsburgh, Pennsylvania},
series = {ICSE '22}
}

@misc{029_pseudocodeExample,
  title = {{Definition of Pseudocode}},
  howpublished = {\url{https://tinyurl.com/3nmkr9nk}},
  note = {{Accessed: 2022-6-20}},
}

@inproceedings{030_CosineSimilarityDefinition,
  title={Cosine similarity scoring without score normalization techniques.},
  author={Dehak, Najim and Dehak, Reda and Glass, James R and Reynolds, Douglas A and Kenny, Patrick and others},
  booktitle={Odyssey},
  pages={15},
  year={2010}
}

@article{031_fastTextOutperformDoc2Vec,
doi = {10.1088/1742-6596/1529/4/042077},
url = {https://dx.doi.org/10.1088/1742-6596/1529/4/042077},
year = {2020},
month = {apr},
publisher = {IOP Publishing},
volume = {1529},
number = {4},
pages = {042077},
author = {S Tiun and U A Mokhtar and S H Bakar and S Saad},
title = {Classification of functional and non-functional requirement in software requirement using Word2vec and fast Text},
journal = {Journal of Physics: Conference Series},
}

@inproceedings{032_Doc2Vec,
  title={Distributed representations of sentences and documents},
  author={Le, Quoc and Mikolov, Tomas},
  booktitle={International conference on machine learning},
  pages={1188--1196},
  year={2014},
  organization={PMLR}
}

@article{033_TFIDF,
  title={An information-theoretic perspective of tf--idf measures},
  author={Aizawa, Akiko},
  journal={Information Processing \& Management},
  volume={39},
  number={1},
  pages={45--65},
  year={2003},
  publisher={Elsevier}
}

@inproceedings{034_HeteroSP,
author = {Phan, Hung and Jannesari, Ali},
title = {Heterogeneous Graph Neural Networks for Software Effort Estimation},
year = {2022},
isbn = {9781450394277},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3544902.3546248},
doi = {10.1145/3544902.3546248},
booktitle = {Proceedings of the 16th ACM / IEEE International Symposium on Empirical Software Engineering and Measurement},
pages = {103–113},
numpages = {11},
keywords = {heterogeneous graph transformer, software effort estimation, graph neural networks},
location = {Helsinki, Finland},
series = {ESEM '22}
}

@article{035_PCA,
  title={Principal component analysis},
  author={Abdi, Herv{\'e} and Williams, Lynne J},
  journal={Wiley interdisciplinary reviews: computational statistics},
  volume={2},
  number={4},
  pages={433--459},
  year={2010},
  publisher={Wiley Online Library}
}

@inproceedings{036_BLEU,
  title={Bleu: a method for automatic evaluation of machine translation},
  author={Papineni, Kishore and Roukos, Salim and Ward, Todd and Zhu, Wei-Jing},
  booktitle={Proceedings of the 40th annual meeting of the Association for Computational Linguistics},
  pages={311--318},
  year={2002}
}

@inproceedings{037_METEOR_Study,
author = {Roy, Devjeet and Fakhoury, Sarah and Arnaoudova, Venera},
title = {Reassessing Automatic Evaluation Metrics for Code Summarization Tasks},
year = {2021},
isbn = {9781450385626},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3468264.3468588},
doi = {10.1145/3468264.3468588},
abstract = {In recent years, research in the domain of source code summarization has adopted data-driven techniques pioneered in machine translation (MT). Automatic evaluation metrics such as BLEU, METEOR, and ROUGE, are fundamental to the evaluation of MT systems and have been adopted as proxies of human evaluation in the code summarization domain. However, the extent to which automatic metrics agree with the gold standard of human evaluation has not been evaluated on code summarization tasks. Despite this, marginal improvements in metric scores are often used to discriminate between the performance of competing summarization models. In this paper, we present a critical exploration of the applicability and interpretation of automatic metrics as evaluation techniques for code summarization tasks. We conduct an empirical study with 226 human annotators to assess the degree to which automatic metrics reflect human evaluation. Results indicate that metric improvements of less than 2 points do not guarantee systematic improvements in summarization quality, and are unreliable as proxies of human evaluation. When the difference between metric scores for two summarization approaches increases but remains within 5 points, some metrics such as METEOR and chrF become highly reliable proxies, whereas others, such as corpus BLEU, remain unreliable. Based on these findings, we make several recommendations for the use of automatic metrics to discriminate model performance in code summarization.},
booktitle = {Proceedings of the 29th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
pages = {1105–1116},
numpages = {12},
keywords = {code summarization, machine translation, automatic evaluation metrics},
location = {Athens, Greece},
series = {ESEC/FSE 2021}
}

@misc{038_cyclomatic_HFCCA,
  title = {{HFCCA: Library for Cyclomatic Metric Measurement}},
  howpublished = {\url{https://tinyurl.com/3bdeh2rx}},
  note = {{Accessed: 2022-6-20}},
}

@INPROCEEDINGS{039_API2Vec,
  author={Nguyen, Trong Duc and Nguyen, Anh Tuan and Phan, Hung Dang and Nguyen, Tien N.},
  booktitle={2017 IEEE/ACM 39th International Conference on Software Engineering (ICSE)}, 
  title={Exploring API Embedding for API Usages and Applications}, 
  year={2017},
  volume={},
  number={},
  pages={438-449},
  doi={10.1109/ICSE.2017.47}}

  @inproceedings{040_CodeBERT,
    title = "{C}ode{BERT}: A Pre-Trained Model for Programming and Natural Languages",
    author = "Feng, Zhangyin  and
      Guo, Daya  and
      Tang, Duyu  and
      Duan, Nan  and
      Feng, Xiaocheng  and
      Gong, Ming  and
      Shou, Linjun  and
      Qin, Bing  and
      Liu, Ting  and
      Jiang, Daxin  and
      Zhou, Ming",
    booktitle = "Findings of the Association for Computational Linguistics: EMNLP 2020",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.findings-emnlp.139",
    doi = "10.18653/v1/2020.findings-emnlp.139",
    pages = "1536--1547",
}

@article{041_Word2Vec,
 title={Efficient estimation of word representations in vector space},
  author={Mikolov, Tomas and Chen, Kai and Corrado, Greg and Dean, Jeffrey},
  journal={arXiv preprint arXiv:1301.3781},
  year={2013}
}

@inproceedings{042_CodeReviewer,
  title={Automating code review activities by large-scale pre-training},
  author={Li, Zhiyu and Lu, Shuai and Guo, Daya and Duan, Nan and Jannu, Shailesh and Jenks, Grant and Majumder, Deep and Green, Jared and Svyatkovskiy, Alexey and Fu, Shengyu and others},
  booktitle={Proceedings of the 30th ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering},
  pages={1035--1047},
  year={2022}
}

@article{043_Code2Vec,
author = {Alon, Uri and Zilberstein, Meital and Levy, Omer and Yahav, Eran},
title = {Code2vec: Learning Distributed Representations of Code},
year = {2019},
issue_date = {January 2019},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {3},
number = {POPL},
url = {https://doi.org/10.1145/3290353},
doi = {10.1145/3290353},
abstract = {We present a neural model for representing snippets of code as continuous distributed vectors (``code embeddings''). The main idea is to represent a code snippet as a single fixed-length code vector, which can be used to predict semantic properties of the snippet. To this end, code is first decomposed to a collection of paths in its abstract syntax tree. Then, the network learns the atomic representation of each path while simultaneously learning how to aggregate a set of them. We demonstrate the effectiveness of our approach by using it to predict a method's name from the vector representation of its body. We evaluate our approach by training a model on a dataset of 12M methods. We show that code vectors trained on this dataset can predict method names from files that were unobserved during training. Furthermore, we show that our model learns useful method name vectors that capture semantic similarities, combinations, and analogies. A comparison of our approach to previous techniques over the same dataset shows an improvement of more than 75%, making it the first to successfully predict method names based on a large, cross-project corpus. Our trained model, visualizations and vector similarities are available as an interactive online demo at http://code2vec.org. The code, data and trained models are available at https://github.com/tech-srl/code2vec.},
journal = {Proc. ACM Program. Lang.},
month = {jan},
articleno = {40},
numpages = {29},
keywords = {Machine Learning, Big Code, Distributed Representations}
}

@article{044_CodeT5,
  title={Codet5: Identifier-aware unified pre-trained encoder-decoder models for code understanding and generation},
  author={Wang, Yue and Wang, Weishi and Joty, Shafiq and Hoi, Steven CH},
  journal={arXiv preprint arXiv:2109.00859},
  year={2021}
}

@article{045_PLBART,
  title={Unified pre-training for program understanding and generation},
  author={Ahmad, Wasi Uddin and Chakraborty, Saikat and Ray, Baishakhi and Chang, Kai-Wei},
  journal={arXiv preprint arXiv:2103.06333},
  year={2021}
}

@article{046_SMTOriginal,
  title={Statistical machine translation},
  author={Lopez, Adam},
  journal={ACM Computing Surveys (CSUR)},
  volume={40},
  number={3},
  pages={1--49},
  year={2008},
  publisher={ACM New York, NY, USA}
}

@article{047_CodeGPT,
  title={Codexglue: A machine learning benchmark dataset for code understanding and generation},
  author={Lu, Shuai and Guo, Daya and Ren, Shuo and Huang, Junjie and Svyatkovskiy, Alexey and Blanco, Ambrosio and Clement, Colin and Drain, Dawn and Jiang, Daxin and Tang, Duyu and others},
  journal={arXiv preprint arXiv:2102.04664},
  year={2021}
}

@inproceedings{048_DLTypeInference,
  title={Deep learning type inference},
  author={Hellendoorn, Vincent J and Bird, Christian and Barr, Earl T and Allamanis, Miltiadis},
  booktitle={Proceedings of the 2018 26th acm joint meeting on european software engineering conference and symposium on the foundations of software engineering},
  pages={152--162},
  year={2018}
}

@article{049_bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}

@inproceedings{050_miceli-barone-sennrich-2017-parallel,
    title = "A Parallel Corpus of Python Functions and Documentation Strings for Automated Code Documentation and Code Generation",
    author = "Miceli Barone, Antonio Valerio  and
      Sennrich, Rico",
    booktitle = "Proceedings of the Eighth International Joint Conference on Natural Language Processing (Volume 2: Short Papers)",
    month = nov,
    year = "2017",
    address = "Taipei, Taiwan",
    publisher = "Asian Federation of Natural Language Processing",
    url = "https://aclanthology.org/I17-2053",
    pages = "314--319",
    abstract = "Automated documentation of programming source code and automated code generation from natural language are challenging tasks of both practical and scientific interest. Progress in these areas has been limited by the low availability of parallel corpora of code and natural language descriptions, which tend to be small and constrained to specific domains. In this work we introduce a large and diverse parallel corpus of a hundred thousands Python functions with their documentation strings ({``}docstrings{''}) generated by scraping open source repositories on GitHub. We describe baseline results for the code documentation and code generation tasks obtained by neural machine translation. We also experiment with data augmentation techniques to further increase the amount of training data. We release our datasets and processing scripts in order to stimulate research in these areas.",
}

==> figTabAlgs/AlgmGetNodes.tex <==
\begin{algorithm}
\SetAlgoLined
    \SetKwFunction{getAllAncestorsFromLeaf}{getAllAncestorsFromLeaf}
    \SetKwInOut{KwIn}{Input}
    \SetKwInOut{KwOut}{Output}
    \KwIn{node: Node, depth: int}
    \KwOut{selectedNode: Node}
    
    $listOfAncestors\gets \getAllAncestorsFromLeaf(node)$
    
    $selectedNode\gets listOfAncestors[listOfAncestors.length-1]$
    
    \If{$listOfAncestors.length>depth$}{

            $selectedNode=listOfAncestors[depth]$

     }
     
    \KwRet{$selectedNode$}
    \caption{Pseudocode of the \textbf{findAncestor()} function}
    \label{asttrans:algm:findAncestor}
\end{algorithm}



==> figTabAlgs/algm2.tex <==
% https://jdhao.github.io/2019/09/21/latex_algorithm_pseudo_code/
% https://tex.stackexchange.com/questions/149162/how-can-i-define-a-foreach-loop-on-the-basis-of-the-existing-forall-loop
\begin{algorithm}[h]
\SetAlgoLined
    \SetKwFunction{getASTForCode}{getASTForCode}
    \SetKwFunction{getLeaves}{getLeaves}
    \SetKwFunction{lookupRepresentation}{lookupRepresentation}
    \SetKwInOut{KwIn}{Input}
    \SetKwInOut{KwOut}{Output}
    \KwIn{candidate: string, depth: int, embModel: Model}
    \KwOut{vectorASTSumRep: Vector}
    
    $astCand\gets \getASTForCode(candidate)$
    
    $listOfLeaves\gets \getLeaves(astCand)$
    
    $seqNodeASTSumReps \gets set()$

    $seqTextASTSumReps \gets []$

    \For{$leaf  \in listOfLeaves$}{
        $nodeRep\gets \lookupRepresentation(leaf,depth)$
        
        \If{$nodeRep \notin seqNodeASTSumReps$}{

            $seqNodeASTSumReps.add(nodeRep)$

            $seqTextASTSumReps.append(getAS(nodeRep))$
         }
    }

    $vectorASTSumRep\gets embModel.getVector(seqTextASTSumReps)$
    
    \KwRet{$vectorASTSumRep$}
    \caption{Algorithm for extracting augmented embedding for code candidate by ASTSum}
    \label{astsum:algm:augmentEmbeddingForCandidates}
\end{algorithm}



==> figTabAlgs/fig_background_icse.tex <==
\begin{figure}
\includegraphics[width=\linewidth]{images/ASTTrans_Background_ECOOP.pdf}
\caption{The Code Search Process by Original Models}
\label{asttrans:fig:originalModels}
\end{figure}

==> figTabAlgs/fig_case234_ecoop.tex <==
\begin{figure*}[h]
    \centering
        \caption{Examples of the cases (query) that ASTTrans outperformed UniXcoder (a), ASTTrans cannot improve for UniXcoder (b) and UniXCoder performed better than UniXcoder augmented with ASTTrans (c)}%
    \label{asttrans:fig:rq2Dimensions}%
    \subfloat[\centering Case 2 in PCSD dataset]{{\includegraphics[width=0.33\linewidth]{images/ASTTrans_GoodCase2.pdf} }}%
    % \qquad
    \subfloat[\centering Case 3 in TLC dataset]{{\includegraphics[width=0.33\linewidth]{images/ASTTrans_BadCase1.pdf} }}%
    % \qquad
    \subfloat[\centering Case 4 in CSN dataset]{{\includegraphics[width=0.33\linewidth]{images/ASTTrans_BadCase2.pdf} }}%
\end{figure*}

==> figTabAlgs/fig_motiv_ecoop_1.tex <==
\begin{figure}
    \centering    
    \caption{Motivation Example with Input Query, Correct Candidate and Incorrect Candidate Returned by UniXcoder}
    \label{asttrans:fig:motiv1}
    \includegraphics[width=\linewidth]{images/ASTTrans_MotivationExample_ECOOP_1.pdf}
\end{figure}

==> figTabAlgs/fig_motiv_ecoop_2.tex <==
\begin{figure}
    \centering    
    \caption{Sub-AST of Line 3 for Code Candidate 1 in Motivation Example}
    \label{asttrans:fig:motiv2}
    \includegraphics[width=\linewidth]{images/ASTTrans_MotivationExample_ECOOP_2.png}
\end{figure}

==> figTabAlgs/fig_motiv_ecoop_3.tex <==
\begin{figure}
    \centering    
    \caption{Sub-AST of Line 3 for Code Candidate 2 in Motivation Example}
    \label{asttrans:fig:motiv3}
    \includegraphics[width=\linewidth]{images/ASTTrans_MotivationExample_ECOOP_3.png}
\end{figure}

==> figTabAlgs/fig_rq2_sen_ecoop.tex <==
\begin{figure}
    \centering
        \caption{RQ2. Percentage of Improvement by MRR by ASTTrans for GraphCodeBERT (blue) and UniXcoder (red) with dimensions from 20 to 768}%
    \label{asttrans:fig:rq2Dimensions}%
    \subfloat[\centering Improvement of MRR for GraphCodeBERT]{{\includegraphics[width=0.48\linewidth]{images/ASTTrans_rq2_dimension_gcb.pdf} }}%
    % \qquad
    \subfloat[\centering Improvement by MRR for UniXcoder]{{\includegraphics[width=0.48\linewidth]{images/ASTTrans_rq2_dimension_unixcoder.pdf} }}%
\end{figure}

==> figTabAlgs/fig_study_notImproveCase.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/ASTTrans_BadCase1.pdf}
    \caption{Example of Cases when ASTTrans cannot improve SOTA approach (in TLC dataset)}
    \label{asttrans:fig:studyNotImproveExample}
\end{figure}

==> figTabAlgs/fig_study_topK.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/ASTTrans_study_topKPercent.pdf}
    \caption{Percentage as number cases at top-k per number of improved cases over four datasets, with $k\in \{1,5,10\}$}
    \label{asttrans:fig:studyTopK}
\end{figure}

==> figTabAlgs/tbl_analysis_ecoop.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[h]
\centering
\caption{Comparison on AST metrics and  similarity metrics  of ASTTrans predict-expected result between the set ASTTrans augmented model outperforms Original models and the set that Original Model performs better (dimension = 768)}
\label{asttrans:tbl:analysisResult}
\begin{tabular}{|l|rrrr|rrrr|}
\hline
                                            & \multicolumn{4}{c|}{\textbf{TLCodesum (7584 queries)}}                                                                              & \multicolumn{4}{c|}{\textbf{CodeSearchNet (19317 queries)}}                                                                         \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}}        & \multicolumn{2}{c|}{\textbf{GCB}}                                     & \multicolumn{2}{c|}{\textbf{UniXcoder}}                               & \multicolumn{2}{c|}{\textbf{GCB}}                                     & \multicolumn{2}{c|}{\textbf{UniXcoder}}                               \\ \hline
\multicolumn{1}{|c|}{\textbf{Metric (Avg)}} & \multicolumn{1}{c|}{\textbf{Aug}} & \multicolumn{1}{c|}{\textbf{Org}} & \multicolumn{1}{c|}{\textbf{Aug}} & \multicolumn{1}{c|}{\textbf{Org}} & \multicolumn{1}{c|}{\textbf{Aug}} & \multicolumn{1}{c|}{\textbf{Org}} & \multicolumn{1}{c|}{\textbf{Aug}} & \multicolumn{1}{c|}{\textbf{Org}} \\ \hline
{\color[HTML]{FF0000} Num. of tokens}       & \multicolumn{1}{r|}{102.30}       & \multicolumn{1}{r|}{101.96}       & \multicolumn{1}{r|}{90.37}        & 101.20                            & \multicolumn{1}{r|}{126.93}       & \multicolumn{1}{r|}{145.01}       & \multicolumn{1}{r|}{125.90}       & 156.87                            \\ \hline
{\color[HTML]{FF0000} Method Call}          & \multicolumn{1}{r|}{5.54}         & \multicolumn{1}{r|}{4.90}         & \multicolumn{1}{r|}{5.06}         & 5.03                              & \multicolumn{1}{r|}{8.16}         & \multicolumn{1}{r|}{7.91}         & \multicolumn{1}{r|}{8.18}         & 8.35                              \\ \hline
{\color[HTML]{FF0000} For statement}        & \multicolumn{1}{r|}{0.24}         & \multicolumn{1}{r|}{0.25}         & \multicolumn{1}{r|}{0.17}         & 0.19                              & \multicolumn{1}{r|}{0.16}         & \multicolumn{1}{r|}{0.23}         & \multicolumn{1}{r|}{0.16}         & 0.28                              \\ \hline
{\color[HTML]{FF0000} Expression statement} & \multicolumn{1}{r|}{4.01}         & \multicolumn{1}{r|}{4.14}         & \multicolumn{1}{r|}{3.53}         & 3.92                              & \multicolumn{1}{r|}{3.80}         & \multicolumn{1}{r|}{4.74}         & \multicolumn{1}{r|}{3.76}         & 5.51                              \\ \hline
{\color[HTML]{FF0000} If statement}         & \multicolumn{1}{r|}{1.53}         & \multicolumn{1}{r|}{1.37}         & \multicolumn{1}{r|}{1.39}         & 1.49                              & \multicolumn{1}{r|}{1.69}         & \multicolumn{1}{r|}{1.84}         & \multicolumn{1}{r|}{1.78}         & 2.05                              \\ \hline
{\color[HTML]{0000FF} CrystalBLEU}          & \multicolumn{1}{r|}{0.48}         & \multicolumn{1}{r|}{0.03}         & \multicolumn{1}{r|}{0.46}         & 0.03                              & \multicolumn{1}{r|}{0.08}         & \multicolumn{1}{r|}{0.01}         & \multicolumn{1}{r|}{0.07}         & 0.01                              \\ \hline
{\color[HTML]{0000FF} Meteor}               & \multicolumn{1}{r|}{0.61}         & \multicolumn{1}{r|}{0.19}         & \multicolumn{1}{r|}{0.60}         & 0.18                              & \multicolumn{1}{r|}{0.24}         & \multicolumn{1}{r|}{0.11}         & \multicolumn{1}{r|}{0.23}         & 0.11                              \\ \hline
                                            & \multicolumn{4}{c|}{\textbf{PCSD (19028 queries)}}                                                                                  & \multicolumn{4}{c|}{\textbf{Funcom (20000 entities)}}                                                                               \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}}        & \multicolumn{2}{c|}{\textbf{GCB}}                                     & \multicolumn{2}{c|}{\textbf{UniXcoder}}                               & \multicolumn{2}{c|}{\textbf{GCB}}                                     & \multicolumn{2}{c|}{\textbf{UniXcoder}}                               \\ \hline
\multicolumn{1}{|c|}{\textbf{Metric (Avg)}} & \multicolumn{1}{c|}{\textbf{Aug}} & \multicolumn{1}{c|}{\textbf{Org}} & \multicolumn{1}{c|}{\textbf{Aug}} & \multicolumn{1}{c|}{\textbf{Org}} & \multicolumn{1}{c|}{\textbf{Aug}} & \multicolumn{1}{c|}{\textbf{Org}} & \multicolumn{1}{c|}{\textbf{Aug}} & \multicolumn{1}{c|}{\textbf{Org}} \\ \hline
{\color[HTML]{FF0000} Num. of tokens}       & \multicolumn{1}{r|}{157.85}       & \multicolumn{1}{r|}{131.72}       & \multicolumn{1}{r|}{151.49}       & 134.49                            & \multicolumn{1}{r|}{40.87}        & \multicolumn{1}{r|}{62.00}        & \multicolumn{1}{r|}{40.51}        & 61.58                             \\ \hline
{\color[HTML]{FF0000} Method Call}          & \multicolumn{1}{r|}{9.62}         & \multicolumn{1}{r|}{6.94}         & \multicolumn{1}{r|}{9.13}         & 7.28                              & \multicolumn{1}{r|}{2.79}         & \multicolumn{1}{r|}{3.70}         & \multicolumn{1}{r|}{2.79}         & 3.66                              \\ \hline
{\color[HTML]{FF0000} For statement}        & \multicolumn{1}{r|}{0.53}         & \multicolumn{1}{r|}{0.37}         & \multicolumn{1}{r|}{0.44}         & 0.32                              & \multicolumn{1}{r|}{0.04}         & \multicolumn{1}{r|}{0.10}         & \multicolumn{1}{r|}{0.05}         & 0.10                              \\ \hline
{\color[HTML]{FF0000} Expression statement} & \multicolumn{1}{r|}{7.96}         & \multicolumn{1}{r|}{5.96}         & \multicolumn{1}{r|}{7.77}         & 5.94                              & \multicolumn{1}{r|}{1.66}         & \multicolumn{1}{r|}{2.81}         & \multicolumn{1}{r|}{1.65}         & 2.77                              \\ \hline
{\color[HTML]{FF0000} If statement}         & \multicolumn{1}{r|}{2.40}         & \multicolumn{1}{r|}{1.60}         & \multicolumn{1}{r|}{2.17}         & 1.51                              & \multicolumn{1}{r|}{0.53}         & \multicolumn{1}{r|}{0.87}         & \multicolumn{1}{r|}{0.52}         & 0.88                              \\ \hline
{\color[HTML]{0000FF} CrystalBLEU}          & \multicolumn{1}{r|}{0.20}         & \multicolumn{1}{r|}{0.01}         & \multicolumn{1}{r|}{0.20}         & 0.01                              & \multicolumn{1}{r|}{0.18}         & \multicolumn{1}{r|}{0.02}         & \multicolumn{1}{r|}{0.17}         & 0.02                              \\ \hline
{\color[HTML]{0000FF} Meteor}               & \multicolumn{1}{r|}{0.38}         & \multicolumn{1}{r|}{0.15}         & \multicolumn{1}{r|}{0.39}         & 0.16                              & \multicolumn{1}{r|}{0.39}         & \multicolumn{1}{r|}{0.16}         & \multicolumn{1}{r|}{0.39}         & 0.16                              \\ \hline
\end{tabular}
\end{table*}

==> figTabAlgs/tbl_analysis_metric_icse.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}
\centering
\caption{Comparison on AST metrics and  similarity metrics  of ASTTrans predict-expected result between the set ASTTrans augmented model outperforms Original models and the set that Original Model performs better (dimension = 768)}
\label{asttrans:tbl:analysisResult}
\begin{tabular}{|l|ll|ll|}
\hline
\multicolumn{1}{|c|}{\textbf{Model}}                                                    & \multicolumn{2}{c|}{\textbf{GCB}}                                     & \multicolumn{2}{c|}{\textbf{UniXcoder}}                               \\ \hline
\multicolumn{1}{|c|}{\textbf{Metric (Avg)}}                                             & \multicolumn{1}{c|}{\textbf{Aug}} & \multicolumn{1}{c|}{\textbf{Org}} & \multicolumn{1}{c|}{\textbf{Aug}} & \multicolumn{1}{c|}{\textbf{Org}} \\ \hline
{\color[HTML]{FF0000} \begin{tabular}[c]{@{}l@{}}Cyclomatic \\ Complexity\end{tabular}} & \multicolumn{1}{l|}{?}            & ?                                 & \multicolumn{1}{l|}{?}            & ?                                 \\ \hline
{\color[HTML]{0000FF} CrystalBLEU}                                                      & \multicolumn{1}{l|}{?}            & ?                                 & \multicolumn{1}{l|}{?}            & ?                                 \\ \hline
{\color[HTML]{0000FF} Meteor}                                                           & \multicolumn{1}{l|}{?}            & ?                                 & \multicolumn{1}{l|}{?}            & ?                                 \\ \hline
\end{tabular}
\end{table}

==> figTabAlgs/tbl_analysis_topK_ecoop.tex <==
\begin{table}[]
\centering
\caption{Analysis on the numbers of cases ASTTrans can improve witth cases that UniXcoder and GCB already suggest the correct candidate in Top-10 and Top-100 candidates (Dimension = 768)}
\label{asttrans:tbl:analysis:topK}
\begin{tabular}{|l|rrr|rrr|}
\hline
\multicolumn{1}{|c|}{\textbf{Model}}   & \multicolumn{3}{c|}{\textbf{GCB}}                                                                       & \multicolumn{3}{c|}{\textbf{UniXcoder}}                                                                           \\ \hline
\multicolumn{1}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{Top-10}} & \multicolumn{1}{c|}{\textbf{Top-20}} & \multicolumn{1}{c|}{\textbf{Total}} & \multicolumn{1}{c|}{\textbf{Top-10}} & \multicolumn{1}{c|}{\textbf{Top-20}} & \multicolumn{1}{c|}{\textbf{Total}} \\ \hline
TLC                                    & \multicolumn{1}{r|}{739}             & \multicolumn{1}{r|}{875}             & 1152                                & \multicolumn{1}{r|}{585}             & \multicolumn{1}{r|}{715}             & 961                                 \\ \hline
CSN                          & \multicolumn{1}{r|}{330}             & \multicolumn{1}{r|}{533}             & 1406                                & \multicolumn{1}{r|}{245}             & \multicolumn{1}{r|}{375}             & 1117                                \\ \hline
Funcom                                 & \multicolumn{1}{r|}{626}             & \multicolumn{1}{r|}{966}             & 2355                                & \multicolumn{1}{r|}{546}             & \multicolumn{1}{r|}{822}             & 2153                                \\ \hline
PCSD                                   & \multicolumn{1}{r|}{1625}            & \multicolumn{1}{r|}{2025}            & 2903                                & \multicolumn{1}{r|}{1402}            & \multicolumn{1}{r|}{1719}            & 2446                                \\ \hline
\end{tabular}
\end{table}

==> figTabAlgs/tbl_example_combineAlgm.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\small
\centering
\caption{Illustration of how the augmented embedding combine with original embedding for GCB and UniXcoder for code search with n1 as query, c1 as correct candidate and c2 as incorrect candidate}
\label{asttrans:tbl:exampleCombineAlgorithm}
\begin{tabular}{|lr|l|lr|l|}
\hline
\multicolumn{1}{|c|}{\textbf{Original}}                                                                                & \multicolumn{1}{c|}{\textbf{Dim1}} & \multicolumn{1}{c|}{\textbf{Dim2}}              & \multicolumn{1}{c|}{\textbf{Augmented}}                            & \multicolumn{1}{c|}{\textbf{Dim3}}        & \multicolumn{1}{c|}{\textbf{Dim4}}               \\ \hline
\multicolumn{1}{|l|}{Org. vector n1}                                                                                    & 0.1                                & \multicolumn{1}{r|}{0.2}                        & \multicolumn{1}{l|}{Aug. vector n1}                                 & 0.01                                      & \multicolumn{1}{r|}{0.02}                        \\ \hline
\multicolumn{1}{|l|}{{\color[HTML]{38761D} \begin{tabular}[c]{@{}l@{}}Org. vector c1 \\ (correct)\end{tabular}}}        & {\color[HTML]{38761D} 0.4}         & \multicolumn{1}{r|}{{\color[HTML]{38761D} 0.4}} & \multicolumn{1}{l|}{{\color[HTML]{38761D} Aug. vector c1}}          & {\color[HTML]{38761D} 0.01}               & \multicolumn{1}{r|}{{\color[HTML]{38761D} 0.02}} \\ \hline
\multicolumn{1}{|l|}{{\color[HTML]{FF0000} \begin{tabular}[c]{@{}l@{}}Org. vector c2 \\ (incorrect)\end{tabular}}}      & {\color[HTML]{FF0000} 0.28}        & \multicolumn{1}{r|}{{\color[HTML]{FF0000} 0.3}} & \multicolumn{1}{l|}{{\color[HTML]{FF0000} Aug. vector c2}}          & {\color[HTML]{FF0000} 0.07}               & \multicolumn{1}{r|}{{\color[HTML]{FF0000} 0.05}} \\ \hline
\multicolumn{2}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}CSM of \\ org. emb.\end{tabular}}}                                     & \multicolumn{1}{c|}{\textbf{Select}}            & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}CSM of \\ aug. emb.\end{tabular}}}            & \multicolumn{1}{c|}{\textbf{Select}}             \\ \hline
\multicolumn{1}{|l|}{{\color[HTML]{38761D} n1, c1}}                                                                    & {\color[HTML]{38761D} 0.949}       &                                                 & \multicolumn{1}{l|}{{\color[HTML]{38761D} n1, c1}}                 & {\color[HTML]{38761D} 1}                  & x                                                \\ \hline
\multicolumn{1}{|l|}{{\color[HTML]{FF0000} n1, c2}}                                                                    & {\color[HTML]{FF0000} 0.959}       & x                                               & \multicolumn{1}{l|}{{\color[HTML]{FF0000} n1, c2}}                 & {\color[HTML]{FF0000} 0.884}              &                                                  \\ \hline
\multicolumn{2}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}CSM of \\ concat. emb.\end{tabular}}}                                                        & \multicolumn{1}{c|}{\textbf{Select}}            & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Combined Score \\\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Select}}             \\ \hline
\multicolumn{1}{|l|}{{\color[HTML]{38761D} \begin{tabular}[c]{@{}l@{}}n1,c1 \end{tabular}}} & {\color[HTML]{38761D} 0.947}       &                                                 & \multicolumn{1}{l|}{{\color[HTML]{38761D} n1,c1}}                  & {\color[HTML]{38761D} 0.954}              & x                                                \\ \hline
\multicolumn{1}{|l|}{{\color[HTML]{FF0000} \begin{tabular}[c]{@{}l@{}}n1,c2 \end{tabular}}}  & {\color[HTML]{FF0000} 0.952}       & x                                               & \multicolumn{1}{l|}{{\color[HTML]{FF0000} n1,c2}}                  & {\color[HTML]{FF0000} 0.951}              &                                                  \\ \hline
\end{tabular}
\end{table}


==> figTabAlgs/tbl_example_nonTerminals.tex <==
\begin{table}[]
\begin{tabular}{|l|l|}
\hline
Candidate & Non-terminal representation                                                                           \\ \hline
Candidate One & \begin{tabular}[c]{@{}l@{}}C\_1\_1 C\_1\_3 C\_1\_8 C\_1\_12 \\ C\_1\_6 C\_1\_10 C\_1\_15\end{tabular} \\ \hline
Candidate Two & \begin{tabular}[c]{@{}l@{}}C\_2\_1 C\_2\_3 C\_2\_5 \\ C\_2\_9 C\_2\_11\end{tabular}                   \\ \hline
\end{tabular}
\caption{Example of sequence of parent nodes of all terminal nodes of Line three of Candidate One and Candidate Two}
\label{asttrans:tbl:exampleOfNonTerminals}
\end{table}

==> figTabAlgs/tbl_rq2_cbc.tex <==
\begin{table}
\centering
\caption{RQ2. Cases by cases comparison over TLC dataset}
\label{asttrans:rq2H2H}
\begin{tabular}{|crrrr|}
\hline
\multicolumn{5}{|c|}{\textbf{Dimension=20}}                                                                                                                                                             \\ \hline
\multicolumn{1}{|c|}{\textbf{ASTTrans}} & \multicolumn{1}{c|}{\textbf{Draw}} & \multicolumn{1}{c|}{\textbf{Original}} & \multicolumn{1}{c|}{\textbf{Outperform}} & \multicolumn{1}{c|}{\textbf{Change}} \\ \hline
\multicolumn{1}{|r|}{2887}              & \multicolumn{1}{r|}{3357}          & \multicolumn{1}{r|}{1340}              & \multicolumn{1}{r|}{38.07\%}             & 55.74\%                              \\ \hline
\multicolumn{1}{|r|}{2843}              & \multicolumn{1}{r|}{3348}          & \multicolumn{1}{r|}{1393}              & \multicolumn{1}{r|}{37.49\%}             & 55.85\%                              \\ \hline
\multicolumn{5}{|c|}{\textbf{Dimension=768}}                                                                                                                                                            \\ \hline
\multicolumn{1}{|c|}{\textbf{ASTTrans}} & \multicolumn{1}{c|}{\textbf{Draw}} & \multicolumn{1}{c|}{\textbf{Original}} & \multicolumn{1}{c|}{\textbf{Outperform}} & \multicolumn{1}{c|}{\textbf{Change}} \\ \hline
\multicolumn{1}{|r|}{1152}              & \multicolumn{1}{r|}{5906}          & \multicolumn{1}{r|}{526}               & \multicolumn{1}{r|}{15.19\%}             & 22.13\%                              \\ \hline
\multicolumn{1}{|r|}{961}               & \multicolumn{1}{r|}{6208}          & \multicolumn{1}{r|}{415}               & \multicolumn{1}{r|}{12.67\%}             & 18.14\%                              \\ \hline
\end{tabular}
\end{table}

==> figTabAlgs/tbl_rq2_mrr.tex <==
\begin{table}[]
\centering
\caption{RQ2. MRR Comparison of code search over TLC dataset}
\label{asttrans:rq2MRR}
\begin{tabular}{|crrrrr|}
\hline
\multicolumn{4}{|c|}{\textbf{Combined Score}}                                                                                      & \multicolumn{2}{c|}{\textbf{Concat. Emb.}}                                 \\ \hline
\multicolumn{6}{|c|}{\textbf{Dimension=20}}                                                                                                                                                                                                     \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}} & \multicolumn{1}{c|}{\textbf{Aug.}} & \multicolumn{1}{c|}{\textbf{Ori.}} & \multicolumn{1}{c|}{\textbf{Imp.}} & \multicolumn{1}{c|}{\textbf{Aug.}} & \multicolumn{1}{c|}{\textbf{Imp.}} \\ \hline
\multicolumn{1}{|l|}{GCB}            & \multicolumn{1}{r|}{53.36\%}          & \multicolumn{1}{r|}{49.71\%}           & \multicolumn{1}{r|}{\textbf{3.65\%}}   & \multicolumn{1}{r|}{49.69\%}          & -0.02\%                                \\ \hline
\multicolumn{1}{|l|}{Unixcoder}      & \multicolumn{1}{r|}{53.58\%}          & \multicolumn{1}{r|}{50.12\%}           & \multicolumn{1}{r|}{\textbf{3.47\%}}   & \multicolumn{1}{r|}{50.56\%}          & 0.44\%                                 \\ \hline
\multicolumn{6}{|c|}{\textbf{Dimension=768}}                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|c|}{\textbf{Model}} & \multicolumn{1}{c|}{\textbf{Aug.}} & \multicolumn{1}{c|}{\textbf{Ori.}} & \multicolumn{1}{c|}{\textbf{Imp.}} & \multicolumn{1}{c|}{\textbf{Aug.}} & \multicolumn{1}{c|}{\textbf{Imp.}} \\ \hline
\multicolumn{1}{|l|}{GCB}            & \multicolumn{1}{r|}{79.15\%}          & \multicolumn{1}{r|}{77.51\%}           & \multicolumn{1}{r|}{\textbf{1.65\%}}   & \multicolumn{1}{r|}{77.51\%}          & 0.00\%                                 \\ \hline
\multicolumn{1}{|l|}{Unixcoder}      & \multicolumn{1}{r|}{80.88\%}          & \multicolumn{1}{r|}{79.72\%}           & \multicolumn{1}{r|}{\textbf{1.16\%}}   & \multicolumn{1}{r|}{79.73\%}          & 0.01\%                                 \\ \hline
\end{tabular}
\end{table}



==> figTabAlgs/tbl_rq3_crossDatasets.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\small
\begin{tabular}{|l|rrrr|}
\hline
                                      & \multicolumn{4}{c|}{\textbf{Target}}                                                                                                                                                                                               \\ \hline
\multicolumn{1}{|c|}{\textbf{Source}} & \multicolumn{1}{c|}{\textbf{TLC}}                           & \multicolumn{1}{c|}{\textbf{CSN}}                           & \multicolumn{1}{c|}{\textbf{Funcom}}                         & \multicolumn{1}{c|}{\textbf{PCSD}}      \\ \hline
TLC                                   & \multicolumn{1}{r|}{\textbf{2.48\%}}                        & \multicolumn{1}{r|}{{\color[HTML]{38761D} \textbf{0.10\%}}} & \multicolumn{1}{r|}{{\color[HTML]{38761D} \textbf{0.03\%}}}  & {\color[HTML]{38761D} \textbf{0.50\%}}  \\ \hline
CSN                                   & \multicolumn{1}{r|}{{\color[HTML]{38761D} \textbf{2.40\%}}} & \multicolumn{1}{r|}{\textbf{0.07\%}}                        & \multicolumn{1}{r|}{{\color[HTML]{38761D} \textbf{0.05\%}}}  & {\color[HTML]{FF0000} \textbf{-0.10\%}} \\ \hline
Funcom                                & \multicolumn{1}{r|}{{\color[HTML]{38761D} \textbf{2.22\%}}} & \multicolumn{1}{r|}{{\color[HTML]{38761D} \textbf{0.06\%}}} & \multicolumn{1}{r|}{\textbf{0.12\%}}                         & {\color[HTML]{FF0000} \textbf{-0.22\%}} \\ \hline
PCSD                                  & \multicolumn{1}{r|}{{\color[HTML]{38761D} \textbf{1.22\%}}} & \multicolumn{1}{r|}{{\color[HTML]{38761D} \textbf{0.02\%}}} & \multicolumn{1}{r|}{{\color[HTML]{FF0000} \textbf{-0.22\%}}} & \textbf{0.91\%}                         \\ \hline
\end{tabular}
\caption{RQ3 Part 4: Results by metric $Average_{EffectMRR}$ of configurations with cross-dataset testing}
\label{asttrans:tbl:rq3_crossDatasets}
\end{table}

==> figTabAlgs/tbl_stat_depth.tex <==
\begin{table}[]
\centering
\begin{tabular}{|l|r|r|}
\hline
\multicolumn{1}{|c|}{\textbf{Rep.}} & \multicolumn{1}{c|}{\textbf{SequenceSize}} & \multicolumn{1}{c|}{\textbf{VocabSize}} \\ \hline
Depth-2                             & 3                                          & 15                                      \\ \hline
Depth-3                             & 11                                         & 72                                      \\ \hline
Depth-4                             & 22                                         & 124                                     \\ \hline
Depth-5                             & 36                                         & 154                                     \\ \hline
Depth-6                             & 49                                         & 160                                     \\ \hline
Depth-7                             & 62                                         & 165                                     \\ \hline
Depth-8                             & 72                                         & 165                                     \\ \hline
Depth-9                             & 80                                         & 165                                     \\ \hline
Code Tokens                         & 100                                        & 267472                                  \\ \hline
\end{tabular}
\caption{Statistics on the size of ASTTrans Representation and Code Tokens' Representation on code snippets of the CAT benchmark \cite{004_CATBenchmark}}
\label{asttrans:studyAST}

\end{table}


==> figTabAlgs/tbl_study_cyclomaticComplexity.tex <==
\begin{table}[]
\small
\begin{tabular}{|l|r|r|r|r|}
\hline
\multicolumn{1}{|c|}{\textbf{Dataset}} & \multicolumn{1}{c|}{\textbf{All}} & \multicolumn{1}{c|}{\textbf{Improve}} & \multicolumn{1}{c|}{\textbf{Same}} & \multicolumn{1}{c|}{\textbf{Decrease}} \\ \hline
TLC                                    & 3.63                              & 3.62                                  & 3.58                               & 3.79                                   \\ \hline
CSN                                    & 4.05                              & 4.18                                  & 4.00                               & 4.50                                   \\ \hline
Funcom                                 & 2.12                              & 1.92                                  & 2.11                               & 2.45                                   \\ \hline
PCSD                                   & 4.30                              & 4.65                                  & 4.14                               & 4.12                                   \\ \hline
\end{tabular}
\caption{The average Cyclomatic Complexity (CC) all cases, improved cases, same-accuracy cases and decreased cases over four datasets of CAT benchmark \cite{004_CATBenchmark}}
\label{asttrans:tbl:cyclomaticComplexity}
\end{table}

==> figTabAlgs/text_caseDefinitions.tex <==
\textbf{Effect in Cases.} In this metric, we want to calculate how the difference between the cases ASTTrans that can improve the rank of a correct candidate for that case and the case that ASTTrans worse the rank of the correct candidate of original embedding models. There are three possibilities for changing the output of the original model for each case: Better (means the rank of the correct candidate by the augmented embedding $rank_{aug}$ is less than the rank of the correct candidate by the original embedding $rank_{org}$), Draw ($rank_{aug}=rank_{org}$) and Worse ($rank_{aug}>rank_{org}$). We call the set of cases that have the result as $Better$ as $Case_{Better}$ and the set of cases with $Worse$ as a result as $Case_{Worse}$. The Formula for calculating the Effect in Cases is defined as follows:
\begin{equation*}
\begin{multlined}
    EffectCases(C,a,o,d)= \\ \frac{|Case_{Better}(C,a,o,d)|-|Case_{Worse}(C,a,o,d)|}{|C|}
    \end{multlined}
    \label{asttrans:eq:definitionEffectCase}
\end{equation*}
Similar to the metric in MRR, the bigger the EffectCases is, the more positive effect that the augmented embedding model can help in improving the SOTA approaches. We use $Average_{EffectCases}(C)$ as the average of EffectCases in four configurations to measure the Effect in Cases ASTTrans can have with all SOTA approaches with different configurations.

